The Design and Analysis of Virtual Network Configuration for a Wireless Mobile ATM Network

This research concentrates on the design and analysis of an algorithm referred to as Virtual Network Configuration (VNC) which uses predicted future states of a system for faster network configuration and management. VNC is applied to the configuration of a wireless mobile ATM network. VNC is built on techniques from parallel discrete event simulation merged with constraints from real-time systems and applied to mobile ATM configuration and handoff. Configuration in a mobile network is a dynamic and continuous process. Factors such as load, distance, capacity and topology are all constantly changing in a mobile environment. The VNC algorithm anticipates configuration changes and speeds the reconfiguration process by pre-computing and caching results. VNC propagates local prediction results throughout the VNC enhanced system. The Global Positioning System is an enabling technology for the use of VNC in mobile networks because it provides location information and accurate time for each node. This research has resulted in well defined structures for the encapsulation of physical processes within Logical Processes and a generic library for enhancing a system with VNC. Enhancing an existing system with VNC is straight forward assuming the existing physical processes do not have side effects. The benefit of prediction is gained at the cost of additional traffic and processing. This research includes an analysis of VNC and suggestions for optimization of the VNC algorithm and its parameters.

==> chap1/philosoph.tex <==
\subsection{Complexity in Self-Predictive Systems}
\label{philo}

The purpose of this section is to ``step out of the box'' 
and view from a few other perspectives the operation of the \ac{VNC} 
algorithm. A perfectly tuned \ac{VNC} system would
have a tolerance for error ($\Theta$) of zero and $\forall t$ 
$GVT(t) > t$, where
$GVT(t)$ is the time into the future that the \ac{VNC} system has
predicted. This means that the system should always be able to
perfectly predict its future. 


==> chap1/proofs.tex <==
\subsection{Proofs in this Thesis}

The more important and frequently used results will be proved in lemmas
and propositions. Each lemma and proposition will be labeled, displayed, then
proved. The proof will consist of the assumptions followed by
the steps of the proof. These proofs
are presented in a hierarchical manner; each step may require another
complete proof which is shown immediately beneath the step
to be proven \cite{LamportProof}. Steps are numbered consecutively
with intermediate step subproof step numbers concatenated with the
current step number. Intermediate step sub-proofs which are many
levels deep may use a short form of numbering, ``$<$n$>$'', where
n refers to the depth of the step. Thus Step $1.2.1.3$ is labeled
Step $<$3$>$3.


==> chap3/la.tex <==
\section{\acl{VNC} Prediction Rate with a Fixed Lookahead}

The prediction rate ($PR$) has been defined in Proposition \ref{splp_rate}.
As the proportion of out-of-order ($X$) and out-of-tolerance ($Y$) messages 
decrease, the prediction rate increases. The prediction rate can naturally
be considered a slope in a graphical representation of \acl{LVT} ($LVT$) and 
real-time ($t$). Clearly, the prediction rate should be greater than
one in order to achieve lookahead ($LA= LVT\index{LVT} - t$). However, $LVT$ does 
not continue to increase at the prediction rate indefinitely. When $LVT$
and $t$ differ by the amount $\Lambda$, the \acl{LP} holds all virtual\index{Virtual Network Configuration!verification}
processing until $t$ reaches $LVT$ as shown in Figure \ref{lookahead}. Thus 
$\Lambda$ is the maximum lookahead and is reached in $\Lambda \cos{(\eta)}$ 
units of real\index{Real}-time, labeled $t$ in Figure \ref{lookahead}. When $\Lambda$
is reached at time $t$, $LVT$ is by definition $\Lambda + t$ time units. 
Therefore, the maximum lookahead ($LA_{max}$) is shown in Equation \ref{la1}. 
A little manipulation results in Equation \ref{la2}.

\begin{figure}[htbp]                                                    
        \centerline{\psfig{file=figures/lookahead.eps,width=3.4in}}          
        \caption{Lookahead as a Function of Prediction Rate and $\Lambda$.}
        \label{lookahead}
\end{figure}

\begin{equation}
\label{la1}
LA_{max} = \Lambda + t - \Lambda \cos{(\eta)}
\end{equation}

\begin{equation}
\label{la2}
LA_{max} = \Lambda (1 - \cos{(\eta - \pi/4)})
\end{equation}

The lookahead is assumed to be a uniformly distributed\index{Distributed} random variable
between 0 and $LA_{max}$. The lookahead probability density function\index{Function} 
is shown in Equation \ref{fla}. The expected lookahead ($E[LA]$) is 
shown in Equation \ref{ela} and is half the value shown in Equation 
\ref{la2} where $\eta$ is $\tan^{-1}(PR)$. Note that $PR$ is defined
as a function\index{Function} of the expected values of $X$ and $Y$.
The speedup\index{Speedup} of a \acl{VNC} over a non-\acl{VNC} system is defined as follows.
If $E[LA] > T_{task}$ then the speedup\index{Speedup} ($C_r$) is the speedup\index{Speedup} in reading 
the cache over the time to execute the task. Otherwise, the speedup\index{Speedup} is 
shown in Equation \ref{su}. Note that $C$ in Equation \ref{su} is the
absolute time to read the cache, not the speedup\index{Speedup} in reading the cache.
The measured versus analytical results are shown in Figure \ref{csu}
with the parameters \analparms Note the analytical values appear
to approach real\index{Real}-time operation of the system faster than the measured 
values. In other words, it appears that the out-of-tolerance message values 
do not have as large a penalty as expected in the analysis. Perhaps
the rollback\index{Rollback} overhead\index{Virtual Network Configuration!overhead} time ($T_{rb}$) is less than expected in the analysis,
or the time warp mechanism within the \acl{VNC} algorithm compensates for 
the out-of-order messages better than expected in the analysis.

\begin{equation}                                                          
\label{fla}                                                     
f_{LA} = {1 \over {\Lambda (1 - \cos{(\tan^{-1}(PR) - \pi/4)})}}
\end{equation}

\begin{eqnarray}
\label{ela}
E[LA] & = \sum_{la=0}^{LA_{max}} f_{LA}\ la & \\
      & = 1/2 {\Lambda (1 - \cos{(\tan^{-1}(PR) - \pi/4)})} &
\end{eqnarray}

\begin{equation}
\label{su}
\alpha \equiv {T_{task} \over {(T_{task} - E[LA]) + C}}
\end{equation}

%\begin{equation}
%\label{sua}
%\alpha \equiv {T_{task} \over {2. - 0.5 \Lambda + T_{task} + 0.5 \Lambda 
%\cos(0.785398 - \tan^{-1}(\lambda_{vm} (\Delta_{vm} - T_{task} - (T_{rb} + 
%T_{task}) E[X] - (\Delta - {1 \over \lambda_{vm}} + T_{rb}) E[Y]}}
%\end{equation}

\begin{figure}[htbp]
        \centerline{\psfig{file=chap3/graphs/cnspeedup.eps,width=3.4in}}
        \caption{Measured versus Analytical Results.}
        \label{csu}
\end{figure}


==> chap5/maisie.tex <==
The simulation has been implemented with Maisie\index{Maisie} \cite{bagrodia}.
Its suitability for this has been demonstrated in the \acl{RDRN}\index{RDRN}
network management and control design and development and in
\cite{Short} to develop a mobile wireless network
parallel simulation\index{Parallel Simulation} environment. The 
parallel simulation\index{Parallel Simulation} 
environment shows a speedup\index{Speedup} over the currently used commercial 
sequential simulation packages.  The environment 
and a set of modules which have been developed for mobile network
simulation are described in \cite{Short}.
%Communicating Sequential Processes
Maisie uses a language which has been influenced by a classic work describing 
the characteristics of a parallel\index{Parallel} programming\index{Parallel Programming}
language structure \cite{Hoare81}. The programming features
developed here are used in many parallel\index{Parallel} programming 
languages\index{Parallel Programming!language} besides Maisie\index{Maisie}\index{Maisie}.
Since every Maisie\index{Maisie} 
entity has a built-in input queue, each \acl{LP} is comprised of three
additional Maisie\index{Maisie} entities:
\begin{itemize}
\item An entity which represents the \acl{PP}\index{PP}
\item An entity for the \acl{LP} state queue\index{State Queue}
\item An entity for the \acl{LP} output message queue\index{Send Queue}
\end{itemize}

There is also a gvt entity\index{Predictive Network Management!gvt entity} for the calculation of Global\index{GVT} 
Time (\acl{GVT}\index{Global Virtual\index{Virtual Network Configuration!verification} Time\index{Time}}). All three of the above 
entities work together to implement Virtual\index{Virtual Network Configuration!verification} Time\index{Time} as described 
in \cite{Jefferson82}. The first entity above, representing the \acl{PP}, 
contains a delay mechanism in order to implement the sliding 
lookahead window\index{Sliding Lookahead Window|see{$\Lambda$}}.
The gvt process should notify all processes to cease forward simulation 
when \acl{GVT} reaches the end of the window. In this version of \acl{VNC}, each \acl{LP}
simply compares its \acf{LVT}\index{LVT} to the current time and holds processing
until current time is back within the lookahead sliding window.

Determination of \acf{GVT}\index{GVT} should be done as defined by
\cite{Lazowaska90}.
This algorithm allows \acl{GVT} to be determined in a message-passing environment
as opposed to the easier case of a shared memory environment. It also
allows normal processing to continue during the \acl{GVT} determination phase.
However, in this implementation\index{Virtual Network Configuration!implementation} each output message is sent to the gvt 
entity as well as to its proper destination. In addition, the gvt entity 
checks all \acl{LP}s for their current \acl{LVT}\index{LVT} and chooses the minimum message send time
and \acl{LVT}\index{LVT} as the current \acl{GVT}. The gvt entity is allowed to execute in parallel\index{Parallel} 
with the other entities in this simulation, it does not stop the other
entities while performing its computation and thus may not always be 
perfectly accurate. However, the results were close enough for the purpose
of these experiments.

State adjustment\index{State Adjustment|see{VNC}} rollback\index{Rollback}s are the 
most critical part of \acl{VNC}.
They are handled in a slightly different fashion from causality\index{VNC!causality}
failure rollback\index{Rollback}s. A state verification\index{Virtual Network Configuration!verification} failure
causes the \acl{LP} state to be corrected at the time of the state 
verification which failed. 
The state, $S_{v}$, has been obtained from the actual device from 
the state adjustment query at time $t_{v}$.
The \acl{LP} rolls back to exactly $t_{v}$ with state, $S_{v}$.
States greater than $t_{v}$ are removed from the state 
queue\index{State Queue}. 
Anti-messages\index{Anti-Message} are sent from the output message queue 
for all messages
greater than $t_{v}$. The \acl{LP} continues forward execution from this 
point.
Note that this implies that the message and state queues cannot
be purged of elements which are older than the \acl{GVT}. Only elements which
are older than real\index{Real} time can be purged.


==> chap5/slpsim.tex <==
\section{Single Processor LP\index{LP} Simulation Results}
\label{slpsim}

The goal of this simplified implementation\index{Virtual Network Configuration!implementation} is experimental validation of 
speedup and lookahead using virtual\index{Virtual Network Configuration!verification} messages and state values which are
subject to becoming out of tolerance due to error. Position information
is cached in each \acl{SLP}.
An actual system of \acl{SLP}s has been built and run on a single processor.
The \acl{SLP}s are copies of the \acl{RDRN} \acl{VNC} \acl{GPS} driving\index{Driving Process}
process. The source \acl{SLP} is the driving\index{Driving Process} process which generates real\index{Real} 
and virtual\index{Virtual Network Configuration!verification} position messages. The system is a linear chain of 
three \acl{SLP}s similar to the \acl{LP}s shown in the bottom of 
Figure \ref{vncpart}. The 
processes communicate via \acl{IPC} message queues and each \acl{SLP} 
receives the \acl{GPS} position message from the \acl{SLP} preceding it in 
the chain.
If the message is a virtual\index{Virtual Network Configuration!verification} message, a predetermined amount of position 
error is added to the location information from the distribution specified 
in Table \ref{lpseq}.
If the message is real\index{Real} the \acl{SLP} determines whether a rollback\index{Rollback} has 
occurred and forwards the message to the successor \acl{SLP} in the chain. 
The final \acl{SLP} in the sequence of \acl{SLP}s records the time and the 
total distance. This \acl{VNC} system is compared to the same set of \acl{LP}s
executing in the same manner except that there are no virtual\index{Virtual Network Configuration!verification} messages or
lookahead.

\begin{table*}[htbp]
\centering
\begin{tabular}{||l|l||}          \hline
\textbf{Parameter } & \textbf{Value} \\ \hline \hline
Initial Location & $(0,0)$     	\\ \hline
Speed            & $0.1$ m/s   	\\ \hline
Direction        & $0.0^o$  	\\ \hline
Tolerance        & $2.0$ m     	\\ \hline
Lookahead        & $300$ s     	\\ \hline
UpdatePeriod     & $2$ s       	\\ \hline
Position Error   & Normal ($\sigma = 0$, $\sigma^2 = 1$) \\ \hline
\end{tabular}
\caption{\label{lpseq} Single Processor Logical Process Model Parameters.}
\end{table*}

The implementation\index{Virtual Network Configuration!implementation} parameters are shown in Table \ref{lpseq}. The speedup\index{Speedup}
is shown by the difference in the predicted distance versus the distance
traveled in a nonVNC system at any point in real\index{Real} time in Figure \ref{seqlpres}.
The system maintained an arbitrarily chosen 300 second $Lookahead$ window 
as shown in Figure \ref{seqlpres}. Distance is simply computed as the 
current speed times the elapsed time and the driving\index{Driving Process} process maintains its
initial direction throughout the simulation. The $UpdatePeriod$
is the virtual\index{Virtual Network Configuration!verification} message generation period in the driving\index{Driving Process} process.
Rollback was caused by 40\% of the virtual\index{Virtual Network Configuration!verification} messages from the driving\index{Driving Process} process.
This compares well with the result from Proposition \ref{prb_hyp} 
which estimates a rollback\index{Rollback} probability of less than or 
equal to 50\%.

\begin{figure*}[htbp]
        \centerline{\psfig{file=figures/vnc.ps,width=4in}}
        \caption{Sequential Logical Process Simulation Results.}
        \label{seqlpres}
\end{figure*}

This simplified orderwire implementation\index{Virtual Network Configuration!implementation} has shown the \acl{SLP} to 
provide significant speedup\index{Speedup} and lookahead using virtual\index{Virtual Network Configuration!verification} messages.
Also the rollback\index{Rollback} overhead\index{Virtual Network Configuration!overhead} caused by state values which are subject 
to becoming out of tolerance due to error has been shown to match
the analytical results.

